Hard-Thresholding Meets Evolution Strategies in Reinforcement Learning

Evolution Strategies (ES) have emerged as a competitive alternative for model-free reinforcement learning, showcasing exemplary performance in tasks like Mujoco and Atari. Notably, they shine in scenarios with imperfect reward functions, making them invaluable for real-world applications where dense reward signals may be elusive. Yet, an inherent assumption in ES, that all input features are task-relevant, poses challenges, especially when confronted with irrelevant features common in real-world problems. This work scrutinizes this limitation, particularly focusing on the Natural Evolution Strategies (NES) variant. We propose NESHT, a novel approach that integrates Hard-Thresholding (HT) with NES to champion sparsity, ensuring only pertinent features are employed. Backed by rigorous analysis and empirical tests, NESHT demonstrates its promise in mitigating the pitfalls of irrelevant features and shines in complex decision-making problems like noisy Mujoco and Atari tasks.

==> chapters/7_rebuttal.tex <==
\clearpage

\textit{Thank you to all three reviewers for their kind and helpful comments. We will make modifications based on these insightful comments. Regarding their concerns:}

\noindent\textit{\textbf{Reviewer \#2.} Section 5.5: How the hard-thresholding ratio affects in complex sparse reward problems?} 
{\color{blue} Results in Figure 3 are all derived from the sparse reward setting, where 90\% of the rewards are set to zero. This setting may increase a bit the bounded variance term $f_\tau$ in our Assumption 2, as the masking operation is random. However, this would not significantly increase $C$ (and thus impede convergence), since $f_\tau$ is calculated for each trajectory rather than each transition.}

\noindent\textit{\textbf{Reviewer \#2.} Intuition for choosing the hard-thresholding ratio? Can this be adaptive?}
{\color{blue} There is indeed a compromise in the choice of the HT ratio: a larger ratio (sparser model) may help convergence by reducing the variance of the ES gradient estimate as we discuss in the paper, but overly large ratios may restrict the policy search space, affecting performance. Therefore, we would advise to the ratio to be based on an \textit{a priori} estimate of the amount of noisy features, or otherwise through some grid parameter search. It may also be adaptive, along training, as you suggested (e.g. one could start with a very large beta to quickly learn very sparse policies, and reduce it gradually to learn complex policies later).}

\noindent\textit{\textbf{Reviewer \#4.} The hard-thresholding ratio parameter $\beta$ can be integrated into Algorithm 1. to replace $k$.} 
{\color{blue}We agree with you and follow your suggestion to revise this paper. The ratio of parameters to be kept, $\beta$, is more convenient for practitioner since it doesn't correlate with the raw feature size. And the number of parameters to be kept, $k$, is more used for theoretical analysis. In fact they can be converted to each other smoothly.}

\noindent\textit{\textbf{Reviewer \#4.}  Add situation with more structured irrelevant signal would be better.}
{\color{blue} Unlike the common practice of cropping an 84x84 region of the image that mainly captures the playing area (DQN NIPS paper by \textit{Volodymyr Mnih}), we use the full screen of the Atari game as input (110x84). This approach includes structured, irrelevant, and real-world-like features, such as the scoreboard and background. As such, we believe our Atari experiments accurately reflect the structured noise setting. We apologize for not mentioning this crucial detail in our submission. (Thank you for the insightful comments!)}


\noindent\textit{\textbf{Reviewer \#4.} How the final sparse policies be deployed?}
{\color{blue} 
% We explore the benefits of the HT operator on NES in terms of managing irrelevant features. However, we will not be discussing its advantage in accelerating inference since it falls outside our research scope.
Our work focuses on using sparsity to manage irrelevant features, not to improve computation. But, indeed, one may just need to store and query only the indices and values of the non-zero elements. This could improve memory consumption, speed up CPU performance, and enhance GPU speed if the sparse GPU kernel is sufficiently efficient and the vectors are sufficiently sparse (sparsity on GPU is usually harder to leverage).}

\noindent\textit{\textbf{Reviewer \#5.} Other approaches, such as feature selection techniques, can be utilized to handle irrelevant features. Why is the HT technique better or more effective than these methods?}
{\color{blue} In the comparison section, we have taken care to include existing NES and RL-family algorithms designed for irrelevant features, such as NES-$L_1$ and ANF-SAC. Techniques beyond HT can also be integrated into the NES algorithm with some code-level adjustments. However, the compatibility of these techniques with the natural gradient is a significant concern. 
Indeed, HT is perhaps the most natural constraint for sparsity: we simply want a given number of parameters to be nonzero.
%It also has the advantages of sparse regularization methods (it is a non-convex regularization method), 
As such, it makes possible to prove the convergence of our method. Finally, compared to other regularizations such as Lasso, MCP, SCAD, etc., it allows to fix $k$ without tuning a regularization strength.}

\noindent\textit{\textbf{Reviewer \#5.}
Why ESs use one-layer linear networks while RLs use three-layer non-linear networks on Mujoco tasks?}
{\color{blue} A one-layer linear structure is a common setting in the Evolutionary Strategy (ES) community, as seen in works like \textit{SGES by Fei-Yu Liu}, \textit{ARS by Horia Mania}. On the other hand, three-layer networks are prevalent in the RL community. We have simply adhered to these established conventions.}

\noindent\textit{\textbf{Reviewer \#5.} How the HT technique performs with respect to a wide range of neural network architecture designs?}
{\color{blue} Indeed, the compatibility between HT and advanced neural network architectures, such as transformers and diffusion models, could be a significant research direction. However, due to our limitations, this paper focuses on the decision-making scenario where MLP and CNNs are most commonly employed.}


\noindent\textit{\textbf{Reviewer \#5.} How useful ES would be in real-world applications where it is infeasible to use 500 CPU cores for training?} 
{\color{blue} The Atari results are derived from runs with 500 CPU hours, following the OpenAI NES paper. The same result can be achieved with fewer CPU cores and extended training time.}


\noindent\textit{\textbf{Reviewer \#5.} Why did the authors not consider applying HT to policy gradient algorithms?}
{\color{blue} There is an algorithm known as ANF-SAC, which we've included in our comparison, that combines HT with the renowned SAC algorithm. However, a theoretical analysis of their compatibility has not been conducted. Furthermore, the combination of HT with the policy gradient algorithm is a topic that has not been explored to our knowledge. We believe that both theoretical analyses could be significant contributions to the RL community. In this study, we consider NES because it has several advantages. It can handle sparse reward settings, is easily parallelizable, and does not require backpropagation(only requires forward propagation).}


\noindent\textit{\textbf{Reviewer \#5.} The authors should highlight more of the technical novelty in their convergence proof, in order for readers to better appreciate the technical difficulty and hence the contribution of the convergence analysis.}
{\color{blue} Indeed, our main contribution is rather on the proofs of Lemma 1 and Lemma 2, which are fully novel to the best of our knowledge.
% , which we then plug into the general framework from [Xu et. al. 2019] to obtain a novel final overall result specific to our setting (Theorem 1). 
We prove Lemma 1 by upper bounding the spectral norm of the  Hessian of $F_{\sigma}$ using properties of the spectral norm for rank-1 matrices and using our assumptions. The proof of Lemma 2 is also novel but perhaps more standard: it builds upon Lemma 4 which is a simple application of our assumptions, and on Lemma 6 which simply shows how averaging several samples reduces the variance (one just needs to be careful and use conditional expectations, since the rollouts $\tau$ are sampled for a given $\veps$). We will add such details in the final manuscript.}

\noindent\textit{\textbf{Reviewer \#5.} I don't understand why the grad of $F(x)$ with respect to $\theta$ can be ignored in A.1.}
{\color{blue}
% For the convenience of the readers, we provide a self-contained derivation of \textit{natural gradients}. 
Since $\bm{x}$ is the variable over which the expectations and integrals are taken over, it is not a function of $\bm{\theta}$, but rather, it is a dummy variable which is integrated over (it spans all $\mathbb{R}^d$, independently of $\bm{\theta}$, which is fixed). $\bm{\theta}$ remains only in $P(\bm{x} | \bm{\theta}, \sigma^2I)$, which is why the gradient $\nabla_{\bm{\theta}}$ only applies to $P(\bm{x} | \bm{\theta}, \sigma^2I)$. Finally, the last line is just a change of variable. We hope this can answer your question regarding A.1.}


==> chapters/related_work.tex <==
Derandomization of random numbers has been previously introduced as antithetic variables for isotropic samples [11] and for the CMA-ES by replacing the sequence of uniform random numbers used for sampling a multivariate normal distribution by scrambling-Halton and Sobol sequences [3, ref. [27]]. However, both approaches can introduce a bias on the step-size update as we will discuss later.


